Fraud Detection in Cryptocurrency Markets with Spatio-Temporal Graph Neural Networks

Technological advancements in cryptocurrency markets have increased accessibility for investors, but concurrently exposed them to the risks of market manipulations. Existing fraud detection mechanisms typically rely on machine learning methods that treat each financial asset (i.e., token) and its related transactions independently. However, market manipulation strategies are rarely isolated events, but are rather characterized by coordination, repetition, and frequent transfers among related assets. This suggests that relational structure constitutes an integral component of the signal and can be effectively represented through graphical means. In this paper, we propose three graph construction methods that rely on aggregated hourly market data. The proposed graphs are processed by a unified spatio-temporal Graph Neural Network (GNN) architecture that combines attention-based spatial aggregation with temporal Transformer encoding. We evaluate our methodology on a real-world dataset comprised of pump-and-dump schemes in cryptocurrency markets, spanning a period of over three years. Our comparative results showcase that our graph-based models achieve significant improvements over standard machine learning baselines in detecting anomalous events. Our work highlights that learned market connectivity provides substantial gains for detecting coordinated market manipulation schemes.

==> Comment.tex <==
\begin{comment}
\section{Anomaly Detection Task}
\label{sec:anomaly-task}
% =========================

We focus on developing an operational machine learning pipeline for detecting pump-and-dump schemes in crypto markets.

The predictive problem considered in this study can be framed as a binary anomaly detection task on an hourly panel of tokens, where one token represents one listed crypto asset.  We denote by \((s,t)\) a symbol--hour pair; the target variable is then a binary label \(y_{s,t} \in \{0,1\}\) indicating whether the hour contains a pump signal:
\[
  y_{s,t} = 
  \begin{cases}
    1, & \text{if at least one pump announcement for token $s$} \\
       & \text{occurs in hour $t$,} \\
    0, & \text{otherwise.}
  \end{cases}
\]

Figure~\ref{fig:temporal} reports a typical pattern for a P\&D for one token in our dataset.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{images/example_pump_ICNBTC.png}
    \caption{$\pm 24$-hour window over the recorded Pump-and-Dump scheme for the ICN token, performed on 2018-04-04. Open price (top right), volume (top left), log-returns (bottom right) and number of trades (bottom left).}
    \label{fig:temporal}
\end{figure}

\subsection{Anomaly perspective}
By construction, the number of positive observations in our dataset is extremely small relative to the size of the panel. Pump events are rare in calendar time, and they are also sparse across tokens. In our dataset, pump hours account for roughly \(0.06\%\) of all observations, so that the vast majority of observed hours represent normal trading conditions. This results in a heavily imbalanced learning problem where naïve classifiers that always predict the negative class can achieve high accuracy but have no practical value for surveillance.

From a conceptual perspective, this class imbalance motivates treating pump hours as \emph{anomalies} in the joint feature space spanned by market activity variables. We formally find empirical evidence to support this view in Section~\ref{sec:data}. At the same time, by construction, we do have explicit labels for a subset of pump episodes. This allows us to evaluate both unsupervised anomaly detectors (which do not use labels during training) and supervised classifiers (which do), and to quantify the incremental value of supervision.

\subsection{Operational objectives}
From the perspective of exchanges and regulators, two monitoring tasks are relevant:

\begin{itemize}
  \item \textbf{Early warning detection.}  
        The objective is to flag, in (near) real time, hours that are likely to contain an ongoing or imminent pump episode so that additional scrutiny can be considered. In this setting, the model must rely on information that is available up to (and including) hour \(t\), and the tolerance for false positives is relatively low because alarms may trigger costly interventions.
  \item \textbf{Retrospective detection.}  
        The objective is to assist ex-post investigations by scanning historical data to identify segments of price and volume that resemble known pump patterns, potentially in the absence of a Telegram record. Here, a higher false-positive rate can be acceptable if it helps uncover previously unseen campaigns.
\end{itemize}

Our experimental design is closer to the preventive setting: we treat each symbol--hour as a candidate pump hour and use only pre-event information when evaluating predictive performance on the held-out test set. Nevertheless, the anomaly scores produced by the unsupervised models can also be exploited in a forensic context to prioritize periods and tokens for manual review.

\subsection{Evaluation metrics}
Given the rarity of the positive class, standard accuracy is uninformative and strongly biased. We instead focus on metrics that explicitly trade off false and true positive predictions:

\begin{itemize}
  \item \textit{Precision}, measuring the fraction of predicted pumps that correspond to true pump hours,
  \item \textit{Recall}, measuring the fraction of true pump hours that are correctly detected,
  \item \textit{F$_1$ score}, defined as the harmonic mean of precision and recall, which penalizes models that perform well on only one of the two dimensions.
\end{itemize}


\section{Data}
\label{sec:data}
The dataset we use was collected from \cite{LaMorgia2020} and includes pump-and-dump schemes detected between July 2017 and January 2021 on the Telegram platform, where 20 groups were analyzed. The dataset includes various securities used to perform a P\&D fraud, listed on 5 exchanges (Bittrex, Yobit, Binance, Cryptopia and Kucoin). In Table~\ref{tab:pump_groups} we report the data regarding the main pumps, the groups and the attacked tokens.

\begin{table}
\centering
\caption{Pump groups and their activity: number of distinct pumps and total attacked tokens. Most active groups are shown at the top.}
\label{tab:pump_groups}
\begin{tabular}{lrrll}
\toprule
group & n\_pumps & n\_tokens & first\_pump & last\_pump \\
\midrule
ATW & 253 & 122 & 2018-01-01 & 2020-10-31 \\
BPF & 230 & 137 & 2018-03-30 & 2021-01-15 \\
CPI & 180 & 112 & 2018-04-14 & 2020-11-09 \\
CPS & 58 & 48 & 2018-06-28 & 2020-11-06 \\
TCG & 46 & 35 & 2017-11-11 & 2021-01-06 \\
C4P & 45 & 34 & 2017-09-21 & 2018-05-12 \\
BPS & 41 & 33 & 2018-01-03 & 2021-01-09 \\
FCS & 36 & 33 & 2018-02-11 & 2018-12-30 \\
CW & 33 & 27 & 2020-01-04 & 2021-01-09 \\
MPG & 32 & 24 & 2018-10-28 & 2020-12-31 \\
BPG & 23 & 10 & 2018-08-08 & 2019-10-03 \\
TWP & 23 & 17 & 2020-07-16 & 2021-01-15 \\
TCC & 22 & 21 & 2017-07-05 & 2021-01-18 \\
LUX & 17 & 17 & 2018-04-09 & 2018-09-22 \\
WCG & 17 & 17 & 2018-05-10 & 2020-01-16 \\
CCS & 14 & 12 & 2018-12-27 & 2020-12-31 \\
PKG & 14 & 13 & 2017-10-23 & 2018-01-25 \\
CCB & 12 & 12 & 2018-09-30 & 2020-03-27 \\
CP & 8 & 5 & 2020-11-27 & 2021-01-13 \\
SE & 5 & 5 & 2018-10-04 & 2019-10-02 \\
\bottomrule
\end{tabular}
\end{table}

In total, 1,100 events have been recorded for 372 tokens affected. The most affected were Raiden Network Token (RNT) and Bread (BRD), with a total of 24 attacks each. Although a large proportion of these tokens are placed on the market for criminal purposes and are somehow de-listed once the fraud is discovered, some of these tokens are still traded, such as RNT and BRD.

Since some events in the raw Telegram dataset are time–stamped with small deviations of one or two minutes, and our predictive exercise is conducted at hourly frequency, we first snap each signal to the nearest full hour (e.g.\ an event at 15:59 is recorded at 16:00).

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/temporal_structure.png}
    \caption{Temporal structure of recorded Pump-and-Dump events, aggregated by token.}
    \label{fig:temporal2}
\end{figure}

Figure~\ref{fig:temporal2} summarizes the temporal structure of the pump signals in the sample. The upper panel reports the monthly number of identified pumps between July 2017 and January 2021. Overall, the monthly profile does not display any clear or persistent seasonal pattern that would justify a formal seasonal decomposition. The lower panel displays the empirical distribution of pumps over the 24 hours of the day. Here a pronounced concentration of events emerges between 16:00 and 18:00, while pumps are extremely rare during the night-time hours. This intraday pattern is economically suggestive. The 16:00–18:00 window closely overlaps with the closing of major US equity markets and the period of highest overlap between US and European trading sessions, when retail participation and overall crypto trading activity are typically elevated. The fact that pump organizers appear to coordinate their activity precisely in these hours is consistent with a behaviour that is far from random: it points to groups that time their campaigns to exploit periods of high liquidity and attention, in line with a deliberately “professional” operating logic rather than purely opportunistic or ad–hoc behaviour.

\subsection{Dataset}
We focus only on pump recorded on the Binance exchange, as we have direct access to market data through the Binance API. To construct the covariates used in the predictive models, we enrich each pump signal with market data around the event. Specifically, for every token we query the Binance API at 1-hour resolution and retrieve aggregated standard OHLCV information (open, high, low, close, traded volume) in a $\pm 3$-day window around the pump time. This design ensures that all features are aligned on the hourly grid implied by Figure~\ref{fig:temporal2}, and that the models are trained on strictly pre-event information when we evaluate their ability to predict pump hours. Complete descriptive statistics for all features, separately for event and non-event observations are reported in Table~\ref{tab:summary-stats} in the Appendix.

To better understand the joint behaviour of the covariates, we compute the Pearson correlation matrix for the full set of numerical features. In Figure~\ref{fig:corr-matrix} we report the correlation matrix. As expected, the four OHLC prices (\texttt{open}, \texttt{high}, \texttt{low}, \texttt{close}) are almost perfectly correlated, with pairwise coefficients often above $0.95$. A similarly tight cluster appears for the volume-related variables (\texttt{volume}, \texttt{quote\_asset\_volume}, \texttt{taker\_buy\_base}, \texttt{taker\_buy\_quote}). This pattern indicates that a large part of the raw feature space is redundant: several variables are essentially different transformations of the same underlying economic quantity.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/corr_matrix.png}
    \caption{Pearson correlation matrix of numerical features
    in the $\pm 3$-day window around pump signals.}
    \label{fig:corr-matrix}
\end{figure}

From a modeling perspective, classical multicollinearity concerns are less critical for tree-based methods such as Isolation Forest and Random Forest, since these methodologies do not rely on matrix inversion and remain numerically stable even when predictors are highly correlated. However, very correlated predictors still have two undesirable effects: (i) they inflate model complexity without adding information, and (ii) they can dilute variable importance measures, since several near-duplicate features compete to explain the same splits. For this reason, before estimating our models, we remove highly correlated features to avoid redundancy and simplify interpretation. In particular, we retain all the features related to volumes, as not all of them are highly correlated, but we maintain only one representative feature for price, specifically we chose the open price. We report the selected set of feature with descriptions in Table~\ref{tab:selected_features} in the Appendix.



\subsection{Market activity around pump events}
Given the nature of pump--and--dump schemes, variables describing trading activity at the time of the signal are of primary interest. We focus on three quantities: trading volume, the number of trades, and the token price level. Because all three are extremely right-skewed, to get a better understanding of the behaviour of these features we work in this section with logarithmic transformations. Figure~\ref{fig:boxplots-activity} reports boxplots of these transformed variables, comparing event observations (the hour in which the signal is issued, \texttt{flag}=1) with non-event observations (\texttt{flag}=0). For both \texttt{log\_volume} and \texttt{log\_num\_trades} we observe a clear location shift: the median and the entire inter-quartile range are substantially higher during pump hours than in the background, while the distribution also becomes more dispersed. This suggests that pumps are associated with both a level effect and a volatility effect in trading activity. The distribution of \texttt{log\_price} exhibits a less dramatic but still visible shift, reflecting the fact that many target tokens are persistently low-priced and that large relative price moves can be generated even at very small absolute price levels.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/trading_activity.png}
    \caption{Boxplots of log-transformed volume, number of trades and price level for event and non-event hours.}
    \label{fig:boxplots-activity}
\end{figure}

This empirical observation has two implications for our modeling strategy. First, from an unsupervised perspective, pump hours occupy a very atypical region of the joint feature space spanned mostly by volume and number of trades, meaning that they look like natural anomalies. This provides empirical support for the use of Isolation Forest as an anomaly-detection tool in Section~\ref{sec:model-families}, where we seek to identify pump-like episodes even outside the labeled sample. Second, from a supervised perspective, the systematic shifts in the distributions of these variables between events and non-events indicate that they carry strong predictive information for the classification task. Random Forests, which are flexible with respect to non-linearities and heavy-tailed predictors, are therefore a natural choice in Section~\ref{sec:model-families}.

\section{Methodology}
\label{sec:model-families}

Starting from the raw dataset, we keep only numeric variables and denote the resulting feature matrix by $X \in \mathbb{R}^{N \times d}$ and the label vector by $y = (y_1,\dots,y_N)^\top$. Before fitting the models we standardize each feature to zero mean and unit variance. The scaler parameters are then fixed and applied to validation and test observations. Although tree-based methods are invariant to monotone transformations, this standardization ensures a consistent pre-processing pipeline and allows for a fair comparison with potential non-tree benchmarks.

\subsection{Design}
To respect the temporal ordering of the data and to mimic a realistic online detection scenario, we adopt a strictly chronological splitting strategy. Let $N$ denote the total number of observations. We partition the index set $\{1,\dots,N\}$ into three contiguous blocks: $\mathcal{I}_{\mathrm{train}} \{1,\dots,n_{\mathrm{train}}\}$,  $\mathcal{I}_{\mathrm{val}}  \{n_{\mathrm{train}}+1,\dots,n_{\mathrm{val}}\}$ and $\mathcal{I}_{\mathrm{test}} \{n_{\mathrm{val}}+1,\dots,N\}$ with $n_{\mathrm{train}} = 0.60\, N $ and $n_{\mathrm{val}} = 0.80\, N$. Thus the earliest $60\%$ of the sample are used for training, the next $20\%$ for model selection and hyperparameter tuning, and the last $20\%$ are reserved as a held-out test set that is accessed only once at the very end of the analysis.

We denote by $\mathcal{I}_{\mathrm{train+val}} = \mathcal{I}_{\mathrm{train}} \cup \mathcal{I}_{\mathrm{val}} = \{1,\dots,n_{\mathrm{val}}\}$ the combined train+validation block. Within $\mathcal{I}_{\mathrm{train+val}}$ we perform expanding-window cross-validation with $K=5$ folds. Let $t_k$ and $u_k$ denote, respectively, the last training index and the last validation index in fold $k$, chosen so that $1 < t_1 < u_1 < \dots < t_K < u_K = n_{\mathrm{val}}$. In fold $k$ the training indices are $\mathcal{I}_{\mathrm{train}}^{(k)} = \{1,\dots,t_k\}$, and the candidate validation indices are $\mathcal{I}_{\mathrm{val}}^{(k)} = \{t_k+1,\dots,u_k\}$. This ensures that the model is always trained on the past and validated on the future, preventing leakage of information from later observations into the training set.

To limit bias from short-range dependence, we impose an additional discretionary \emph{embargo} of five observations (5 hours) after the last training index $t_k$. Concretely, we remove the first five elements of the candidate validation set and retain only
\[
\mathcal{I}_{\mathrm{val}}^{(k)} = \{\, i \in \{t_k+1,\dots,u_k\} : i > t_k + 5 \,\}.
\]
This approach reduces the short-lag autocorrelation effect during training and yields a more conservative estimate of out-of-sample performance. This methodology is explained in details in \cite{LopezDePrado2018}.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/fl_cv.png}
    \caption{Expanding–window cross-validation with an embargo period in the train+validation block. In each fold $k$, the model is trained on the contiguous set of past observations $\mathcal{I}_{\mathrm{train}}^{(k)}$ (black), followed by a fixed-length embargo window that is excluded from evaluation, and then validated on the subsequent block $\mathcal{I}_{\mathrm{val}}^{(k)}$ (grey). The training and validation windows move forward over time, and $n_{\mathrm{val}}$ marks the end of the train+validation block.}
    \label{fig:boxplots-activity}
\end{figure}

For each hyperparameter configuration of a given model we perform cross-validation as follows. In each fold $k$ we fit the pre-processing and the model on $X_{\mathcal{I}_{\mathrm{train}}^{(k)}}$ and $y_{\mathcal{I}_{\mathrm{train}}^{(k)}}$ only; we obtain scores or predicted probabilities on the corresponding validation set $X_{\mathcal{I}_{\mathrm{val}}^{(k)}}$ and store them in an out-of-fold (OOF) score vector of length $|\mathcal{I}_{\mathrm{train+val}}|$. Pooling these OOF scores across folds produces, for each observation in the train+validation block, a model prediction computed without using its own label for training. This is the closest analogue to repeatedly rolling the model forward in time. We then select a scalar threshold $\tau$ on the OOF scores that maximizes the F$_1$ score. This procedure yields, for each model family, a tuple consisting of (i) the best-performing hyperparameter configuration, (ii) the corresponding OOF scores, and (iii) a single global decision threshold $\tau^\star$.

Once the best configuration is selected, we refit the model on the full train+validation set $\mathcal{I}_{\mathrm{train+val}}$ using the pre-processing learned on this block, we evaluate it once on the test set $\mathcal{I}_{\mathrm{test}}$ and finally produce test metrics.



\subsection{Supervised classification}
The supervised benchmark is a Random Forest (RF) classifier \cite{breiman2001random} trained on the labeled binary outcome $y_t \in \{0,1\}$. RFs are ensembles of decision trees constructed on bootstrap samples of the training data; at each split a random subset of features is considered, which decorrelates the trees and improves generalization. The final prediction is obtained by majority vote (for class labels) or by averaging the class probabilities across trees. In our setting RFs are attractive for several reasons. First, they can capture non-linear interactions between features such as volume, number of trades, BTC-related covariates and cross-sectional indicators without requiring an explicit parametric specification. Second, they are relatively robust to heavy tails and skewed distributions, which were clearly visible in the EDA. Third, RFs provide measures of variable importance that can be related back to the economic interpretation of the features.

All models are initialized with a fixed random seed and trained with parallelization enabled. For each hyperparameter combination we perform expanding-window cross-validation with embargo as described. We tune the model using the hyperparameter reported in Table~\ref{tab:hparam-grid} in the Appendix.

\subsection{Unsupervised anomaly detection}
To complement the supervised benchmark, we also consider an unsupervised anomaly-detection approach based on the Isolation Forest (IF) model \cite{liu2008isolation}. IF is specifically designed for situations where anomalous observations are rare and located in sparse regions of feature space. The main idea is to isolate points by repeatedly partitioning the feature space with random splits: anomalies, being more isolated, tend to require fewer splits to be separated from the rest of the data, leading to shorter path lengths in the corresponding trees. 

Formally, an IF consists of an ensemble of random isolation trees. Each tree is built by recursively selecting a feature at random and then choosing a split value uniformly within the range of that feature in the current node. The process continues until either all points in a node are identical or a maximum tree depth is reached. The anomaly score of an observation is a decreasing function of its average path length across the trees: unusually short paths correspond to high anomaly scores.

In contrast to the RF, the IF is trained using only the feature vectors $X$, without access to the labels $y$ inside each fold. Labels are used only at the evaluation stage to select hyperparameters and a decision threshold, making this a semi-supervised evaluation of a fundamentally unsupervised model. 

Similarly, we tune the model using the hyperparameters reported in Table~\ref{tab:hparam-grid} in the Appendix and we run the same expanding-window cross-validation with embargo as for the RF. The contamination parameter, which in the standard IF is used to define a built-in threshold on the anomaly scores, is fixed at $0.5$ and ignored when converting scores to labels; we treat the raw decision scores as a ranking and calibrate the final threshold externally.


% ------------------------------------------------
\section{Results}
\label{sec:results}

We compare the out-of-sample performance of the unsupervised Isolation Forest and the supervised Random Forest classifiers on the held-out test set. To assess the robustness of the conclusions with respect to random initialization and bootstrap variation, we repeat the entire training, hyperparameter tuning and evaluation pipeline for nine different random seeds.

Table~\ref{tab:results-main} reports, for each model family, the precision, recall and F$_1$ score computed for the two approaches and for each seed, with the overall mean and standard deviation (in parentheses). The RF clearly dominates the IF across all metrics. On average, the RF achieves an F$_1$ score of $0.709$ with relatively small variability across seeds, while the IF reaches an average F$_1$ of $0.576$. In absolute terms, the RF improves precision by about $0.11$ points and recall by about $0.15$ points relative to the IF, indicating that the supervised model is able to recover a substantially larger fraction of pump events at a lower false alarm rate. The standard deviations are modest for both models, which suggests that the ranking induced by the expanding-window calibration is reasonably stable.

\begin{table}[htbp]\centering
\caption{Test-set precision, recall and F$_1$ across random seeds.}
\label{tab:results-main}
\begin{tabular}{lrrrrrr}
\toprule
& \multicolumn{3}{c}{Isolation Forest} & \multicolumn{3}{c}{Random Forest} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Seed & P & R & F$_1$ & P & R & F$_1$ \\
\midrule
11 & \textbf{0.598} & 0.527 & 0.560 & 0.627 & 0.742 & 0.680 \\
22 & 0.514 & 0.591 & 0.550 & \textbf{0.714} & 0.645 & 0.678 \\
33 & 0.526 & 0.645 & 0.580 & 0.659 & 0.871 & \textbf{0.750} \\
44 & 0.472 & 0.720 & 0.570 & 0.624 & \textbf{0.892} & 0.735 \\
55 & 0.527 & 0.624 & 0.571 & 0.628 & 0.871 & 0.730 \\
66 & 0.591 & 0.591 & 0.591 & 0.604 & 0.871 & 0.714 \\
77 & 0.486 & 0.742 & 0.587 & 0.628 & 0.871 & 0.730 \\
88 & 0.469 & 0.742 & 0.575 & 0.638 & 0.871 & 0.736 \\
99 & 0.500 & \textbf{0.763} & \textbf{0.604} & 0.596 & 0.667 & 0.629 \\
\midrule
Mean     & 0.520 & 0.661 & 0.576 & 0.635 & 0.811 & 0.709 \\
Std.\ dev.& 0.047 & 0.084 & 0.016 & 0.035 & 0.098 & 0.039 \\
\bottomrule
\end{tabular}
\end{table}

From a fraud-detection perspective, these results highlight a clear trade-off between model assumptions and predictive performance. The unsupervised IF, which does not use label information during training, already identifies pump hours as systematic anomalies in the feature space and attains a non-trivial F$_1$ around $0.576$. We conclude that the IF provides a realistic baseline for scenarios in which labels are scarce or unavailable. However, when reliable labels are available, the RF substantially increase both precision and recall.

\subsection{Explainability}
\label{sec:explainability}

We focus on the interpretation of the best detector, which is the Random Forest classifier with seed 33.  Specifically, we compute (i) the standard RF Gini-based feature importance and (ii) SHAP (SHapley Additive exPlanations) values \cite{lundberg2017unified} using the TreeSHAP algorithm on the held-out test set. For each observation, SHAP values decompose the deviation of the predicted pump probability from a reference baseline into additive contributions of each feature. The mean absolute SHAP value across test observations then provides a global importance measure that is directly comparable across features.

In Figure~\ref{fig:feat_imp} and Figure~\ref{fig:feat_shap} we report the standard Random Forest Gini importances and the global SHAP-based importances. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{images/rf_imp.png}
    \caption{Random Forest feature importances.}
    \label{fig:feat_imp}
\end{figure}

We observe that \texttt{num\_trades} is by far the most influential predictor in both rankings. The RF splits most frequently on this variable and SHAP attributes to it the largest average contribution (in absolute value) to the predicted pump probability. This confirms that the intensity of transaction flow, rather than price level per se, is the main signal the model associates with pump-and-dump episodes. Variables that proxy traded value and aggressive buying, such as \texttt{quote\_asset\_volume} and \texttt{taker\_buy\_quote}, also receive large importance scores. We further observe that \texttt{hour\_of\_day} appears as a non-negligible predictor, especially in the SHAP plot, where it ranks second. This complements the descriptive evidence in Section~\ref{sec:data}, where we observed a pronounced concentration of events between 16:00 and 18:00. The model therefore learns a temporal ''fixed effect'': conditional on similar trading patterns, hours in the late afternoon are assigned a higher pump probability. BTC-wide indicators (\texttt{price\_BTC} and \texttt{volume\_BTC}) have very low importance in both metrics. Once token-specific order-flow and volume are controlled for, the marginal contribution of market-wide conditions to the classification decision is small. The \texttt{open} price and raw \texttt{volume} of the token are also of moderate importance only.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{images/shap_imp.png}
    \caption{Random Forest SHAP values.}
    \label{fig:feat_shap}
\end{figure}

Finally, the absolute magnitude of SHAP values is small for all features. This is mechanically due to the extreme class imbalance: the baseline pump probability is close to zero, so even features with high relative importance can change the predicted probability by only a few percentage points. Rather, pump detection emerges from the joint effect of several activity-related covariates, with \texttt{num\_trades}, \texttt{quote\_asset\_volume}, \texttt{taker\_buy\_quote} and \texttt{hour\_of\_day} providing the dominant signals.
\end{comment}
%  



%% As agreed, we don't need this section anymore.
\begin{comment}
% =========================
\section{Selected Real-World Cases}
% =========================
\subsection{SafeMoon (2021–2025)}
The SafeMoon token (SFM) was launched in early 2021 as a cryptocurrency marketed with promises of steady gains, as its promotional slogan "Safely to the moon" suggested. SafeMoon rise is an ideal example for a case study of pump-and-dump methodologies.

Starting in March 2021, SafeMoon’s market capitalization reached the multi-billion dollar range in just two months, only to crash once investors learned the truth. The SEC litigation release \cite{SEC-Complaint-2023} quantifies this rise as roughly a 55,000\% gain from mid-March to April 20, 2021, followed by a near-50\% drop after the liquidity misrepresentation was exposed.  

The case actually revolves around two main frauds: a pump-and-dump scheme with aggressive marketing through celebrity tweets and a general misleading mechanism. Regarding the latter, the cryptocurrency mechanism was never fully and honestly disclosed to investors. The founders claimed that half of each 10\% transaction fee (5\%) would go to a securely locked liquidity pool; as stated in their white paper, the company repeatedly assured investors that these funds would be locked for four years as a security measure \cite{SEC-Complaint-2023}. In reality, however, the developers retained special tokens as liquidity providers (LPs) that allowed them to withdraw all accumulated assets at will \cite{SEC-Complaint-2023}. Therefore, the alleged lock-up was a sham, as those with access to these LPs “repeatedly looted” the pool, siphoning off millions of dollars for personal use, including expenses such as cars, houses, and travel \cite{SEC-PR-2023-229}. When the public discovered that the pool was not actually protected, the value of the token plummeted following complaints that eventually led to the company's bankruptcy in 2023.

Evidently, the company did not act transparently towards investors and, for this reason alone, can already be considered fraudulent. Added to this is the dissemination of misleading statements regarding the functioning of the token and the subsequent implementation of a pump-and-dump scheme, which contributed significantly to the artificial appreciation of SFM's value. SafeMoon executives hired celebrities as spokespersons and conducted aggressive marketing campaigns that fueled interest and drove up the price. This led to a class action lawsuit \cite{MerewhuadervSafeMoon2022}, alleging that these “misleading promotions and celebrity endorsements” artificially inflated demand, while the founders secretly sold large quantities of their own tokens at the peak. The SEC also reports that the CEO himself was responsible for “wash trading”\footnote{Wash trading is a manipulation tactic in which a person trades with themselves or an accomplice to falsify market volume.}, repeatedly buying and selling through a personal account to give the impression of intense trading activity \cite{SEC-PR-2023-229}. In effect, insiders promoted and inflated the token, then dumped their holdings to realize profits, leaving ordinary investors with losses when prices collapsed. Between 2021 and 2022, these operations were commonplace; these celebrities promoted the token via Twitter and then sold at the peak, effectively perpetrating a continuous form of a pump-and-dump scheme. 

Overall, regulators describe SafeMoon’s actions as a “massive fraudulent scheme” that misled investors with false claims and deceptive practices \cite{SEC-Complaint-2023}. Both the SEC complaint and investor lawsuits allege that the team violated securities laws by misrepresenting the locked liquidity and by trading on inside information. In the end, SafeMoon’s rise was clearly unsustainable: the token architecture was abused to line insiders’ pockets, and late buyers suffered heavy losses. This case highlights the risks associated with speculative digital assets and demonstrates that, especially in the case of publicly traded tokens where transparency is lacking, pump-and-dump schemes typically thrive, leading to regulatory action only when the scheme is exposed and to significant losses for retail investors.

\subsection{Operation Token Mirrors (DoJ/FBI, Oct.\ 9, 2024)}
``This investigation, the first of its kind, identified numerous fraudsters in the cryptocurrency industry. Wash trading has long been outlawed in the financial markets, and cryptocurrency is no exception. These are cases where an innovative technology -- cryptocurrency -- met a century old scheme -- the pump-and-dump. The message today is, if you make false statements to trick investors, that's fraud. Period. Our Office will aggressively pursue fraud, including in the cryptocurrency industry,'' said Acting United States Attorney Joshua Levy.

On Oct.\ 9, 2024, prosecutors in Boston unsealed criminal charges against eighteen individuals and entities for widespread fraud and manipulation in crypto markets. The action targeted both token issuers and four crypto market makers accused of delivering wash trading at scale. Authorities reported four guilty pleas (with another agreed), three arrests in Texas, the United Kingdom, and Portugal, seizures exceeding \$25 million in cryptocurrency, and the deactivation of multiple trading bots used to fabricate millions of dollars of volume across roughly 60 tokens.

According to charging documents, several token teams combined false statements with sham trades to manufacture the appearance of organic demand, then sold into the artificially inflated prices. The largest token ecosystem named in the filings, Saitama, reportedly reached a multi\hbox{-}billion\hbox{-}dollar market value at its peak while leadership allegedly coordinated small, multi\hbox{-}wallet buys to create the illusion of massive buys and new holders, later engaging market makers to sustain activity on venues such as BitMart, LBank, and XT.com. Related projects cited include Robo Inu and VZZN.

A central feature of the investigation, named Operation Token Mirrors, was an FBI-led honeypot. The Bureau created a fictitious company and token, NexFundAI, and used them to observe in real time how market makers proposed and executed pump-and-dump schemes. Three companies—ZM Quant, CLS Global, and MyTrade—and their employees have been charged with wash trading and/or conspiracy to engage in wash trading on behalf of NexFundAI, while a fourth company, Gotbit, its CEO, and two directors have been indicted in a parallel case. In candid sales conversations, a market-making executive described the business model in secondary markets as finding “other buyers in the community, people you don't know or care about,” because “we have to make [other buyers] lose money to make a profit.” These remarks sum up the logic behind the scheme: profits for insiders are structurally financed by losses imposed on uninformed market participants.

\subsection{From Pump-and-Dump to Rug Pulls: SQUID (2021)}
In November 2021, the SQUID token---marketed as a ``play-to-earn'' coin inspired by Netflix's \textit{Squid Game}---collapsed in what appeared to be a classic \emph{rug pull} fraud. A rug pull is similar to a pump-and-dump scheme, with one major difference regarding the exit strategy. After raising funds via token sales or by attracting liquidity, perpetrators of a rug pull intentionally appropriate investor funds by withdrawing custodial assets (e.g., liquidity or treasury), disabling or constraining selling possibilities, and/or abruptly abandoning the project, thereby rendering the asset effectively worthless for outside holders. The SQUID case displayed \emph{protocol/contract} constraints (anti-sell/blacklisting logic and discretionary controls) that prevented exit for ordinary holders, followed by a rapid liquidity removal by insiders, in line with a standard rug pull pattern. As widely reported by the BBC (Nov.\ 2, 2021), the token's price surged by thousands of percent within days (from roughly \$0.01 to over \$2{,}800) before crashing by \(\approx 99.99\%\). Holders complained they could not sell due to contract-level restrictions, while the promoters allegedly withdrew proceeds (estimated around \$3.38M) and disappeared.





\begin{table}[htbp]
\centering
\caption{Description of the main market features in the hourly dataset.}
\label{tab:selected_features}
\begin{tabular}{p{0.22\linewidth} p{0.72\linewidth}}
\toprule
Feature & Description \\
\midrule

\texttt{open} &
Opening price of the token in the corresponding 1-hour interval, expressed in the quote currency (e.g.\ USDT). \\[0.5em]

\texttt{volume} &
Total amount of the base asset exchanged during the 1-hour interval (sum of all buy and sell executions in base units). \\[0.8em]

\texttt{quote\_asset\_volume} &
Total traded amount expressed in the quote asset during the 1-hour interval (e.g.\ the value of trades in USDT). \\[0.8em]

\texttt{num\_trades} &
Count of all executed trades during the hour. \\[0.8em]

\texttt{taker\_buy\_base} &
Volume of base asset bought by takers. Takers are traders who place market orders that immediately execute against existing limit orders. When a taker buys, the counterparty is necessarily a maker selling.  
\\[1.0em]

\texttt{taker\_buy\_quote} &
Value of taker buy trades expressed in the quote asset.  
This is simply the monetary value of \texttt{taker\_buy\_base} measured in quote units rather than base units. \\[0.8em]

\texttt{price\_BTC} &
Opening price of Bitcoin (BTC) in the same 1-hour interval. \\[0.8em]

\texttt{volume\_BTC} &
Total Bitcoin traded volume during the same 1-hour interval. \\[0.8em]

\texttt{hour\_of\_day} &
Hour of the day (0--23). \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}[htbp]\centering
\caption{Hyperparameter grids for Random Forest (RF) and Isolation Forest (IF).}
\label{tab:hparam-grid}
\begin{tabular}{lll}
\toprule
Hyperparameter & RF grid & IF grid \\
\midrule
Number of trees $n_{\mathrm{estimators}}$
  & $\{200, 400, 600, 800, 1000, 2000\}$ 
  & $\{200, 400, 600, 800, 1000, 2000\}$ \\
Maximum depth $\max_{\mathrm{depth}}$
  & $\{\text{None}, 10, 20, 30, 40\}$ 
  & -- \\
Minimum samples per leaf $\min_{\mathrm{samples\_leaf}}$
  & $\{1, 5, 10, 15\}$ 
  & -- \\
Feature subsampling $\max_{\mathrm{features}}$
  & $\{\sqrt{d}\}$ 
  & $\{0.3, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0\}$ \\
Subsample size $\max_{\mathrm{samples}}$
  & -- 
  & $\{\text{auto}, 512, 1024\}$ \\
Class weights
  & $\{\text{None}, \text{balanced}\}$ 
  & -- \\
Bootstrap
  & default (= True) 
  & fixed to False \\
\bottomrule
\end{tabular}
\end{table}


\end{comment}
